Distributed Weighted Parameter Averaging for SVM Training on Big Data

Two popular approaches for distributed training of SVMs on big data are parameter averaging and ADMM. Parameter averaging is efficient but suffers from loss of accuracy with increase in number of partitions, while ADMM in the feature space is accurate but suffers from slow convergence. In this paper, we report a hybrid approach called weighted parameter averaging (WPA), which optimizes the regularized hinge loss with respect to weights on parameters. The problem is shown to be same as solving SVM in a projected space. We also demonstrate an $O(\frac{1}{N})$ stability bound on final hypothesis given by WPA, using novel proof techniques. Experimental results on a variety of toy and real world datasets show that our approach is significantly more accurate than parameter averaging for high number of partitions. It is also seen the proposed method enjoys much faster convergence compared to ADMM in features space.

==> background1.tex <==
\subsection{Background}
\label{sec:background}
\vspace{-2mm}
Given a training dataset $S = \{(\mathbf{x}_i,y_i) : i=1,\cdots,ML$, $y_i \in \{-1,+1\},\mathbf{x_i \in \mathbf{R}^d}\}$, the linear SVM problem \cite{vapnik98} is given by: 
\begin{equation}
\label{eq:nondistribsvm}
\min_{\mathbf{w}} \lambda\|\mathbf{w}\|_2^2+\frac{1}{m}\sum_{i=1}^{ML} loss(\mathbf{w};(\mathbf{x}_i,y_i)),
\end{equation}
where, $\lambda$ is the regularization parameter and
% and it trades-off the thickness of the margin i.e., the distance of the support vectors from the separating hyperplane and the weight given to the hinge loss.
the hinge loss is defined as $loss(\mathbf{w};(\mathbf{x}_i,y_i)) = max(0,1-y_i\mathbf{w}^T\mathbf{x}_i)$.
The separating hyperplane is given by the equation $\mathbf{w}^T\mathbf{x} + b = 0$. Here we include the bias $b$ within
$\mathbf{w}$ by making the following transformation, $\mathbf{w} = \left[\mathbf{w}^T,b\right]^T$ and $\mathbf{x}_i = \left[\mathbf{x}_i^T,1\right]^T$

%Given this definition of the SVM problem, our aim is to find an approximation for the SVM parameter $\mathbf{w}$ under distributed setting. This problem is of particular interest when the volume of training data is so large that it cannot be handled efficiently in a single computer, or, the data is distributed at different sites and it is not possible to gather the entire data at a single site due to some reason. The SVM problem under the distributed settings is as follows;
 
 
%%%%%%%%%%%%%%  DISTRIBITED SVM PROBLEM STATEMENT - START %%%%%%%%%%%%%%%%%
%The distributed version of the SVM problem may be stated as follows;%as given by Boyd et al.(section 8.2). 
The above SVM problem can be posed to be solved in a distributed manner, which is interesting when the volume of training data is too large to be effectively stored and processed on a single computer.
%Let the dataset is partitioned by rows as,$\mathbf{X} = \{\mathbf{X}_1,\cdots,\mathbf{X}_M\}$ and $\mathbf{y} = \{y_1,\cdots,y_M\}$
Let the dataset be which is partitioned into $M$ partitions ($\mathcal{S}_m,\ m=1,\dots,M$), each having $L$ datapoints. Hence, $\mathcal{S}=\mathcal{S}_1\cup,\dots,\cup\mathcal{S}_M$, where $\mathcal{S}_m=\{(\mathbf{x}_{ml},y_{ml})\},l=1,\dots,L$.
%Hence, $N=ML$.  Let $\mathbf{X}_m$ denote the data matrix for $m^{th}$ partition with row $i$ as $\mathbf{x}_i^T$.
% Also, let $\mathbf{y}_m,\ m=1,\dots,M$ denote the vector of labels for datapoints in $\mathcal{S}_m$. Let $\mathbf{A}_m \in \vect{R}^{l \times d} = - \diag{\mathbf{y}_m} \mathbf{X}_m$ denote the coefficient matrix in the $m^{th}$ partition.
Under this setting, the SVM problem (Eqn \ref{eq:nondistribsvm}), can be stated as:
\begin{align}
 & \min_{\mathbf{w}_m,\mathbf{z}}  \sum_{m=1}^M \sum_{l=1}^{L} loss(\mathbf{w}_{m};(\mathbf{x}_{ml},y_{ml})) + r(\mathbf{z}) \label{eq:distribprob} \\
 & \mbox{s.t.} \mathbf{w}_{m} - \mathbf{z} = 0, m=1,\cdots,M,\ l=1,\dots,L \nonumber
\end{align}
where $loss()$ is as described above and $r(\mathbf{z}) = \lambda\| \mathbf{z} \|^2$.% $r(z)=\lambda\|\hat{\mathbf{W}} \bs{\beta}\|^2$.
This problem is solved in \cite{boyd11} using ADMM (see section \ref{sec:distalgo}). %This problem can also be solved using distributed sub-gradient descent.
%This problem can be solved using various methods, such as, Alternating Direction Method of Multipliers, Distributed Gradient Descent etc. These methods, are iterative and takes multiple passes to arrive at the solution.
 %%%%%%%%%%%%%%  DISTRIBITED SVM PROBLEM STATEMENT - END %%%%%%%%%%%%%%%%%
 
%\newcommand{\argmin}{\mbox{argmin}} 
 
Another method for solving distributed RLM problems, called parameter averaging (PA), was proposed by Mann et. al. \cite{mann09}, in the context of {\it conditional maximum entropy} model. Let 
$\hat{\mathbf{w}}_m = \argmin_{\mathbf{w}} \frac{1}{L}\sum_{l=1}^{L} loss(\mathbf{w};\mathbf{x}_{ml},y_{ml}) + \lambda \|\mathbf{w}\|^2\ ,\ m=1,\dots,M$ be the standard SVM solution obtained by training on partition $\mathcal{S}_m$.
Mann et al. \cite{mann09} suggest the approximate final parameter to be the arithmetic mean of the parameters learnt on individual partitions, ($\hat{\mathbf{w}}_m$). Hence:
\begin{align}
 & \mathbf{w}_{PA} = \frac{1}{M}\sum_{m=1}^M \hat{\mathbf{w}}_m \label{eq:PA}
\end{align}
Zinekevich et al. \cite{zinekevich10} have also suggested a similar approach where $\hat{\mathbf{w}}_m$'s are learnt using SGD.
% parameter averaging on , where they .
We tried out this approach for SVM. Note that assumptions regarding differentiability of loss function made in \cite{boyd11} can be relaxed in case of convex loss function with an appropriate definition of bregmann divergence using sub-gradients (see section \ref{sec:stability}). The results (reported in section \ref{sec:exp}) show that the method fails to perform well as the number of partitions increase.
% where $M = \mbox{number of partitions and}$ and $\mathbf{w}_m$ is the parameter learnt using $m^{th}$ partition.
This drawback of the above mentioned approach motivated us to propose the weighted parameter averaging method described in the next section.% that has the following advantages. Firstly, is should be faster computationally when the number of features is much larger as compared to the number of partitions and accuracy remains much more stable with increase in the number of sites for a fixed size of the training dataset, compared to the work of ~\cite{NIPS2009_0345}. In this work, we propose an alternative method to alleviate some of the drawbacks.


==> distalgo1.tex <==
\subsection{Distributed algorithms for WPA using ADMM}
\label{sec:distalgo}
\vspace{-2mm}

In the distributed setting, we assume the presence of a central (master) computer which stores and updates the final hypothesis. The partitions of training set $\mathcal{S}_1,\dots,\mathcal{S}_M$ are distributed to $M$ (slave) computers, where the local optimizations are performed. The master needs to communicate to slaves and vice versa. However, no communication between slaves is necessary. Thus, the underlying networks has a star topology, which is also easily implemented using Big data platforms like Hadoop \cite{hadoop}.

Let $\bm{\gamma}_m$, for $m = 1,\cdots,M$ be the weight values at the $M$ different nodes and $\bm{\beta}$ be the value of the weights at the central server. The formulation given in eqn. \ref{eq:nondistopt} can be written as:
\begin{align}
 & \min_{\mathbf{\gamma}_m,\mathbf{\beta}}  \frac{1}{ML} \sum_{m=1}^M \sum_{l=1}^{L} loss(\hat{W}\bm{\gamma}_m;\mathbf{x}_{ml},y_{ml}) + r(\bs{\beta}) \label{eq:distribprob} \\
 & \mbox{s.t.}\hspace{0.5cm} \bs{\gamma}_{m} - \bs{\beta} = 0,\hspace{0.25cm} m=1,\cdots,M,\ \nonumber
\end{align}
where $r(\bs{\beta})=\lambda\|\hat{\mathbf{W}} \bs{\beta}\|^2$. The augmented lagrangian for the above problem is:
$L(\bs{\gamma}_m,\bs{\beta},\bs{\lambda})=\frac{1}{ML}\sum_{m=1}^M \sum_{l=1}^{L} loss(\hat{W}\bm{\gamma}_m;\mathbf{x}_{ml},y_{ml}) + r(\bs{\beta})
 + \sum_{i=1}^M\frac{\rho}{2}\|\bs{\gamma}_m - \bs{\beta}\|^2 + \sum_{i=1}^M\bs{\lambda}_m^T(\bs{\gamma}_m - \bs{\beta})$, where $\bm{\psi}_{m}$ is the lagrange multiplier vector corresponding to $m^{th}$ constraint.
% and  The aim is to achieve  consensus of the value of $\bm{\beta}$ and $\bm{\gamma}$s at the differ nodes. In order to solve this consensus problem, we used the  method of \textit{Alternating Direction Method of Multipliers(ADMM)}.
%\subsection{Alternating Direction Method of Multipliers}
%This problem can be solved using ADMM technique described in \cite{boyd11}. 
Let $\mathbf{A}_m \in \vect{R}^{L \times d} = - \diag{\mathbf{y}_m} \mathbf{X}_m \hat{W} $.% denote the coefficient matrix in the $m^{th}$ partition.
Using results from \cite{boyd11}, the ADMM updates for solving the above problem can derived as:
%the distributed version of our weighted averaging problem is given in algorithm ~\ref{algo:dspt}.
%\begin{align}
% & \bm{\gamma}_m^{k+1} := \argmin_{\bm{\gamma}_m}(1^T (A_m\bm{\gamma}_m + 1)_+ + \rho/2 \| \bm{\gamma}_m^k - \bm{\beta}^k - u_m^k \|_2^2) \\
% & \bm{\beta}^{k+1} := (\hat{W}^T\hat{W} + M\rho I_m)^{-1} M\rho(\overline{\bm{\gamma}}^{k+1} + \overline{u}^{k+1}) \\
% & u_m^{k+1} = u_m^{k} + \bm{\gamma}_m^{k+1} - \bm{\beta}^{k+1}.
%\end{align}
\begin{align}
 & \bs{\gamma}_{m}^{k+1} := \argmin_{\bs{\gamma}} (loss(\mathbf{A}_i \bs{\gamma} ) + (\rho/2)\|\bs{\gamma}_ml - \bs{\beta}^k + \mathbf{u}_{m}^k\|_2^2) \\
 & \bs{\beta}^{k+1} := \argmin_{\bs{\beta}}(r(\bs{\beta}) + (M\rho/2)\|\bs{\beta}-\overline{\bs{\gamma}}^{k+1}-\overline{\mathbf{u}}^k\|_2^2) \\
 & \mathbf{u}_{m}^{k+1} = \mathbf{u}_{m}^{k} + \bs{\gamma}_m^{k+1} - \bs{\beta}^{k+1}.
\end{align}
where, $\mathbf{u}_m = \frac{1}{\rho}\bs{\lambda_m}$, $\overline{\bm{\gamma}} = \frac{1}{M}\sum_{m=1}^M\bm{\gamma}_m$ and $\overline{\mathbf{u}} = \frac{1}{M}\sum_{m=1}^M\mathbf{u}_m$
and the superscript $k$ denotes the iteration counts. Algorithm \ref{algo:dspt} describes the full procedure.
% $\bs{\gamma}_m^k$, for $m = 1,\cdots,M$ are the parameter values at the $M$ different nodes and $\bs{\beta}$ is the value of the parameter at the central server.
{\small
\begin{algorithm}[h]
\caption{Distributed Weighted Parameter Averaging (DWPA)}
\label{algo:dspt}
\SetAlgoLined
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Partitioned datasets $\mathcal{S}_m$, SVM parameter learnt for each partition $\mathbf{\hat{w}}_m, \forall m={1,\cdots, M}$}
\Output{Optimal weight vector $\bm{\beta}$}
\BlankLine
Initialize $\bm{\beta} = \mathbf{1}, \bm{\gamma}_m=\mathbf{1}, \mathbf{u}_m=\mathbf{1}, \forall m \in \{1,\cdots,M\}$\;
\While{$k < T$}{ 
\tcc{\emph{Executed on slaves}}
\For{$m\leftarrow 1$ \KwTo $M$}{
$\bm{\gamma}_m^{k} := \argmin_{\bm{\gamma}_m}(1^T (A_m\bm{\gamma}_m + 1)_+ + \rho/2 \| \bm{\gamma}_m^{k-1} - \bm{\beta}^{k-1} - \mathbf{u}_m^{k-1} \|_2^2)$
}
\BlankLine
\tcc{\emph{Executed on master}}
$\bm{\beta}^{k} := (\hat{W}^T\hat{W} + M\rho I_m)^{-1} M\rho(\overline{\bm{\gamma}}^{k} + \overline{\mathbf{u}}^{k-1})$ ~\label{beta:update} \\
% \tcc{\emph{For each partition get the value of $\bm{u}_m^{k}$}}
\For{$m\leftarrow 1$ \KwTo $M$}{
$\mathbf{u}_m^{k} = \mathbf{u}_m^{k-1} + \bm{\gamma}_m^{k} - \bm{\beta}^{k}$ ~\label{u:update}
}
}
%\vspace{-5mm}
\end{algorithm}
}

A heuristic called \textit{overrelaxation} \cite{boyd11} is ofter used for improving the convergence rate of ADMM. For overrelaxation, the updates for $\bm{beta}^{k}$ (line \ref{beta:update} and $\mathbf{u}_m^{k}$ (line \ref{u:update}) are obtained by replacing $\overline{\bm{\gamma}}^{k}$ with $\bm{\hat{\gamma}}_m^{k} = \alpha\times\bm{\gamma}_m^{k} + (1-\alpha)\times\bm{\beta}^{k-1}$, in algorithm \ref{algo:dspt}. We implemented this heuristic for both DSVM and DWPA. We call them accelarated DSVM (DSVMacc) and accelarated DWPA (DWPAacc).



==> intro1.tex <==
\section{Introduction}
\label{sec:intro}

With the growing popularity of Big Data platforms \cite{hadoop} for various machine learning and data analytics applications \cite{mann09, zinekevich10}, distributed training of Support Vector Machines (SVMs)\cite{vapnik98} on Big Data platforms have become increasingly important. Big data platforms such as Hadoop \cite{hadoop} provide simple programming abstraction (Map Reduce), scalability and fault tolerance at the cost of distributed iterative computation being slow and expensive \cite{mann09}. Thus, there is a need for SVM training algorithms which are efficient both in terms of the number of iterations and volume of data communicated per iteration.

The problem of distributed training of support vector machines (SVM) \cite{forero10} in particular, and distributed regularized loss minimization (RLM) in general \cite{boyd11, mann2009}, has received a lot of attention in the recent times. Here, the training data is partitioned into $M$-nodes, each having $L$ datapoints. Parameter averaging (PA), also called ``mixture weights'' \cite{mann09} or ``parallelized SGD'' \cite{zinkevich10}, suggests solving an appropriate RLM problem on data in each node, and use average of the resultant parameters. Hence, a single distributed iteration is needed. However, as shown in this paper, the accuracy of this approach reduces with increase in number of partitions. Another interesting result described in \cite{mann09} is a bound of $O(\frac{1}{ML})$ on the stability of the final hypothesis, which results in a bound on generalization error of the algorithm.

Another popular approach for distributed RLM is \textit{alternating direction method of multipliers} (ADMM) \cite{boyd11,forero10}. This approach tries to achieve consensus between parameters at different nodes while optimizing the objective function. It achieves optimal performance irrespective of the number of partitions. However, a this approach needs  many distributed iterations. Also, %size of problem solved in each iteration and 
number of parameters to be communicated among machines per iteration is same as the dimension of the problem. This can be $\sim$ millions for some practical datasets, e.g. webspam \cite{libsvmdata}.

In this paper, we propose a hybrid approach which uses weighted parameter averaging and proposes to learn the weights in a distributed manner from the data. %While weighted parameter averaging has also been mentioned in \cite{mann09}, the authors have used equal weightage $(\frac{1}{m},\dots,\frac{1}{m})$, as they did not propose a method for learning the weights.
We propose a novel SVM-like formulation for learning the weights of the weighted parameter averaging (WPA) model. The dual of WPA turns out to be same as SVM dual, with data projected in a lower dimensional space. We propose an ADMM \cite{boyd11} based distributed algorithm (DWPA), and an accelerated version (DWPAacc), for learning the weights.

Another contribution is a $O(\frac{1}{ML})$ bound on the stability of final hypothesis leading to bound on generalization error of the algorithm. This requires a novel proof technique as both the original parameters and the weights are solutions to optimization problems. Empirically, we show that that accuracy of parameter averaging degrades with increase in the number of partitions. Experimental results on real world datasets show that DWPA and DWPAacc achieve better accuracies than PA as the number of partitions increase, while requiring lower number of iterations and time per iteration compared to ADMM. %weighted parameter averaging performs much better than parameter averaging on both toy and real life datasets.

%\textbf{Related Work}: B

==> intro2.tex <==
\section{Introduction}
\label{sec:intro}

With the growing popularity of Big Data platforms \cite{hadoop} for various machine learning and data analytics applications ~\cite{mann09, zinekevich10}, distributed training of Support Vector Machines (SVMs)\cite{vapnik95} on Big Data platforms have become increasingly important. Big data platforms such as Hadoop \cite{hadoop} provide simple programming abstraction (Map Reduce), scalability and fault tolerance at the cost of distributed iterative computation being slow and expensive \cite{mann09}. Thus, there is a need for SVM training algorithms which are efficient both in terms of the number of iterations and volume of data communicated per iteration.

The problem of distributed training of support vector machines (SVM) \cite{forero10} in particular, and distributed regularized loss minimization (RLM) in general \cite{boyd11, mann09}, has received a lot of attention in the recent times. Here, the training data is partitioned into $M$-nodes, each having $L$ datapoints. Parameter averaging (PA), also called ``mixture weights'' \cite{mann09} or ``parallelized SGD'' \cite{zinekevich10}, suggests solving an appropriate RLM problem on data in each node, and use average of the resultant parameters. Hence, a single distributed iteration is needed. However, as shown in this paper, the accuracy of this approach reduces with increase in number of partitions. Another interesting result described in \cite{mann09} is a bound of $O(\frac{1}{ML})$ on the stability of the final hypothesis, which results in a bound on generalization error of the algorithm.

Another popular approach for distributed RLM is \textit{alternating direction method of multipliers} (ADMM) ~\cite{boyd11,forero10}. This approach tries to achieve consensus between parameters at different nodes while optimizing the objective function. It achieves optimal performance irrespective of the number of partitions. However, a this approach needs  many distributed iterations. Also, %size of problem solved in each iteration and 
number of parameters to be communicated among machines per iteration is same as the dimension of the problem. This can be $\sim$ millions for some practical datasets, e.g. webspam \cite{libsvmdata}.

In this paper, we propose a hybrid approach which uses weighted parameter averaging and proposes to learn the weights in a distributed manner from the data. %While weighted parameter averaging has also been mentioned in \cite{mann09}, the authors have used equal weightage $(\frac{1}{m},\dots,\frac{1}{m})$, as they did not propose a method for learning the weights.
We propose a novel SVM-like formulation for learning the weights of the weighted parameter averaging (WPA) model. The dual of WPA turns out to be same as SVM dual, with data projected in a lower dimensional space. We propose an ADMM \cite{boyd11} based distributed algorithm (DWPA), and an accelerated version (DWPAacc), for learning the weights.

Another contribution is a $O(\frac{1}{ML})$ bound on the stability of final hypothesis leading to bound on generalization error of the algorithm. This requires a novel proof technique as both the original parameters and the weights are solutions to optimization problems. Empirically, we show that that accuracy of parameter averaging degrades with increase in the number of partitions. Experimental results on real world datasets show that DWPA and DWPAacc achieve better accuracies than PA as the number of partitions increase, while requiring lower number of iterations and time per iteration compared to ADMM. %weighted parameter averaging performs much better than parameter averaging on both toy and real life datasets.

%\textbf{Related Work}: B

==> wpa_1.tex <==
\subsection{Weighted parameter averaging (WPA)}
\label{sec:formulation}
\vspace{-2mm}

The parameter averaging method uses uniform weight of $\frac{1}{M}$ for each of the $M$ components. One can conceive a more general setting where the final hypothesis is a weighted sum of the parameters obtained on each partition: $\mathbf{w} = \sum_{m=1}^M\beta_m\mathbf{\hat{w}_m}$, where $\mathbf{\hat{w}_m}$ are as defined above and $\beta_m \in \RR, m=1,\dots,M$. Thus, $ \bm{\beta} = [\beta_1,\cdots,\beta_M]^T = [\frac{1}{M},\dots,\frac{1}{M}]$ achieves the PA setting. Note that Mann et al. \cite{mann09} proposed $\bm{\beta}$ to be in a simplex. However, no scheme was suggested for learning an appropriate $\bm{\beta}$.

Our aim is to find the optimal set of weights $\bm{\beta}$ which attains the lowest regularized loss.
%that integrates the SVM parameters ${\mathbf{w}_i,b_i}$, $i = 1,\cdots,M$ learnt from disjoint partitioning of the dataset at $M$ different nodes to give a single parameter, that approximates the SVM parameter learnt from the entire dataset at a single node.
%The entire dataset is partitioned into $M$ partitions and  each partition of the entire dataset is used to learn a different parameter $\hat{\mathbf{w}_m}$, where, $m = {1,\cdots,M}$. 
Let $\mathbf{\hat{W}} = [\hat{\mathbf{w}_1},\cdots,\hat{\mathbf{w}_M}]$ so that $\mathbf{w} = \mathbf{\hat{W}}\bm{\beta}$.
The regularized loss minimization problem is stated as follows;
\begin{align}
&  \min_{\bm{\beta}, \mathbf{\xi}} \lambda \|\mathbf{\hat{W}} \bm{\beta}\|^2 + \frac{1}{ML} \sum_{m=1}^{M} \sum_{i=1}^{l} \xi_{mi} \label{eq:nondistopt} \\
& \mbox{\textbf{subject to:} } y_{mi}(\bm{\beta}^T \mathbf{\hat{W}}^T x_{mi}) \geq 1 - \xi_{mi}, \hspace{0.25cm} \forall i,m \nonumber \\
& \hspace{2cm} \xi_{mi} \geq 0, \hspace{0.25cm} \forall m=1,\dots,M,\ i=1,\dots,l \nonumber
\end{align}
Note that, here the optimization is only w.r.t. $\bm{\beta}$ and $\xi_{m,i}$. $\hat{\bm{W}}$ is a pre-computed parameter. Next we can derive the dual formulation by writing the lagrangian and eliminating the primal variables. The Lagrangian is given by:
\begin{align}
%\label{lagrangian}
\scriptsize{
 \mathcal{L}(\bm{\beta}, \xi_{mi}, \alpha_{mi}, \mu_{mi}) = \lambda \|\mathbf{\hat{W}} \bm{\beta}\|^2 + \frac{1}{ML} \sum_{m,i}\xi_{mi} + \sum_{m,i} \alpha_{mi} ( y_{mi}(\bm{\beta}^T W^T x_{mi}) - 1 + \xi_{mi}) - \sum_{m,i} \mu_{mi} \xi_{mi}
 } \nonumber
\end{align}
%Given the Lagrangian $L$ as in equation ~\ref{lagrangian}, the dual of the problem is obtained by minimizing the Lagrangian with respect to $\beta$ and $\xi_{mi}$, where  $i \in {1,\cdots,l}$ and $m \in {1,\cdots,M}$.
Differentiating the Lagrangian w.r.t. $\bm{\beta}$ and equating to zero, we get:
\begin{equation}
\label{beta:dual}
\bm{\beta} = \frac{1}{2\lambda}(\mathbf{\hat{W}}^T\mathbf{\hat{W}})^{-1}(\sum_{m,i}\alpha_{mi}y_{mi}\mathbf{\hat{W}}^Tx_{mi})
\end{equation}
Differentiating $\mathcal{L}$ w.r.t. $\xi_{mi}$ and equating to zero, $\forall i \in {1,\cdots, L}$ and $\forall m \in {1,\cdots,M}$, implies $\frac{1}{ML} - \alpha_{mi} - \mu_{mi} = 0 $.
Since $\mu_{mi} \geq 0$ and $\alpha_{mi} \geq 0$, $0 \leq \alpha_{mi} \leq \frac{1}{ML} $. 
Substituting the value of $\bm{\beta}$ in the Lagrangian $\mathcal{L}$, we get the dual problem:
\begin{align}
& \min_{\bm{\alpha}}\mathcal{L}(\bm{\alpha}) = \sum_{m,i}\alpha_{mi} - \frac{1}{4\lambda}\sum_{m,i}\sum_{m',j}\alpha_{mi}\alpha_{m'j}y_{mi}y_{m'j}(x_{mi}^T\mathbf{\hat{W}}(\mathbf{\hat{W}}^T\mathbf{\hat{W}})^{-1}\mathbf{\hat{W}}^Tx_{m'j}) \label{dual:formula}\\
& \mbox{\textbf{subject to:}  } 0 \leq \alpha_{mi} \leq \frac{1}{ML}\ \ \ \forall i \in {1,\cdots, L}, m \in {1,\cdots,M} \nonumber
\end{align}
Note that this is equivalent to solving SVM using the projected datapoint $(\mathcal{H}x_{mi},y_{mi})$, instead of $(x_{mi},y_{mi})$, where $\mathcal{H}=\mathbf{\hat{W}}(\mathbf{\hat{W}}^T\mathbf{\hat{W}})^{-1}\mathbf{\hat{W}}^T$, which is the projection on column space of $\mathbf{\hat{W}}$. Hence the performance of the method is expected to depend on size and orientation of the column space of $\mathbf{\hat{W}}$. Next, we describe distributed algorithms for learning $\bm{\beta}$

